Practical Boolean Decomposition for Delay-driven LUT Mapping

Ashenhurst-Curtis decomposition (ACD) is a decomposition technique used, in particular, to map combinational logic into lookup tables (LUTs) structures when synthesizing hardware designs. However, available implementations of ACD suffer from excessive complexity, search-space restrictions, and slow run time, which limit their applicability and scalability. This paper presents a novel fast and versatile technique of ACD suitable for delay optimization. We use this new formulation to compute two-level decompositions into a variable number of LUTs and enhance delay-driven LUT mapping by performing ACD on the fly. Compared to state-of-the-art technology mapping, experiments on heavily optimized benchmarks demonstrate an average delay improvement of 12.39%, and area reduction of 2.20% with affordable run time. Additionally, our method improves 4 of the best delay results in the EPFL synthesis competition without employing design-space exploration techniques.

==> tables/structures.tex <==
\begin{table*}[th]
\setlength\tabcolsep{1.5pt}
\centering
\caption{Comparison of delay-driven LUT mapping and multiple ACD-based mapping into ``66'' cascade structures.}
\footnotesize
\label{tab:structures}
\begin{tabularx}{\textwidth}{lXrrrrXrrrrXrrrrXrrrr}
\toprule
\textbf{Benchmark} &  & \multicolumn{4}{c}{\textbf{dch; if -K 6}} &  & \multicolumn{4}{c}{\textbf{dch; if -S 66}~\cite{Ray_2012}} &  & \multicolumn{4}{c}{\textbf{dch; if -J 66 1-SS}} &  & \multicolumn{4}{c}{\textbf{dch; if -J 66 M-SS}} \\
                   &  & LUTs    & Edges    & Delay   & Time (s)   &  & LUTs      & Edges     & Delay    & Time(s) &  & LUTs       & Edges      & Delay     & Time(s)  &  & LUTs      & Edges      & Delay     & Time(s)   \\ \cmidrule{1-1} \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21} 
adder              &  & 363     & 1433     & 22      & 0.18       &  & 352       & 1521      & 13       & 0.85    &  & 356        & 1552       & 13        & 0.52     &  & 354       & 1550       & 13        & 0.83      \\
bar                &  & 1664    & 9344     & 4       & 0.44       &  & 1664      & 8320      & 3        & 1.34    &  & 1664       & 8320       & 3         & 0.75     &  & 1664      & 8320       & 3         & 0.78      \\
div                &  & 8618    & 32394    & 406     & 6.62       &  & 11555     & 46558     & 266      & 34.87   &  & 11071      & 45711      & 251       & 27.54    &  & 11298     & 47587      & 248       & 30.87     \\
hyp                &  & 58393   & 239097   & 1864    & 5.43       &  & 65987     & 274992    & 1144     & 270.03  &  & 65352      & 274000     & 1082      & 161.75   &  & 65175     & 273434     & 1076      & 183.77    \\
log2               &  & 9712    & 43562    & 58      & 17.05      &  & 12813     & 59950     & 42       & 73.19   &  & 12526      & 58798      & 40        & 54.03    &  & 12409     & 59528      & 39        & 71.87     \\
max                &  & 831     & 3804     & 14      & 0.37       &  & 1177      & 6162      & 9        & 1.77    &  & 1113       & 5448       & 9         & 1.31     &  & 1113      & 5448       & 9         & 1.44      \\
multiplier         &  & 7383    & 34137    & 36      & 6.01       &  & 8898      & 42566     & 25       & 46.10   &  & 8861       & 42005      & 25        & 31.27    &  & 8645      & 43556      & 24        & 36.15     \\
sin                &  & 1928    & 8445     & 30      & 1.31       &  & 2620      & 12074     & 22       & 12.45   &  & 2461       & 11125      & 21        & 9.39     &  & 2400      & 10977      & 21        & 13.17     \\
sqrt               &  & 7515    & 29573    & 663     & 4.17       &  & 9510      & 37809     & 423      & 42.21   &  & 9109       & 37396      & 403       & 24.86    &  & 9441      & 38373      & 398       & 32.31     \\
square             &  & 4122    & 17319    & 23      & 1.98       &  & 4299      & 19677     & 15       & 11.75   &  & 4290       & 19843      & 14        & 8.07     &  & 4299      & 19972      & 14        & 12.65     \\
arbiter            &  & 1833    & 8982     & 6       & 1.64       &  & 2000      & 9481      & 4        & 2.71    &  & 1992       & 9834       & 4         & 2.53     &  & 1992      & 9834       & 4         & 2.50      \\
cavlc              &  & 137     & 707      & 4       & 0.13       &  & 125       & 645       & 3        & 0.49    &  & 124        & 639        & 3         & 0.43     &  & 110       & 565        & 2         & 0.54      \\
ctrl               &  & 30      & 133      & 2       & 0.07       &  & 28        & 131       & 2        & 0.08    &  & 28         & 133        & 1         & 0.09     &  & 28        & 133        & 1         & 0.09      \\
dec                &  & 287     & 684      & 2       & 0.09       &  & 512       & 2304      & 1        & 0.11    &  & 512        & 2304       & 1         & 0.12     &  & 512       & 2304       & 1         & 0.12      \\
i2c                &  & 312     & 1360     & 3       & 0.16       &  & 327       & 1530      & 2        & 0.49    &  & 319        & 1478       & 2         & 0.41     &  & 306       & 1433       & 2         & 0.45      \\
int2float          &  & 52      & 258      & 3       & 0.08       &  & 51        & 257       & 2        & 0.17    &  & 42         & 216        & 2         & 0.17     &  & 38        & 191        & 2         & 0.20      \\
mem\_ctrl          &  & 11037   & 48812    & 18      & 10.24      &  & 11666     & 52725     & 13       & 59.20   &  & 11247      & 51109      & 13        & 48.04    &  & 11019     & 50726      & 13        & 56.43     \\
priority           &  & 178     & 725      & 6       & 0.11       &  & 175       & 761       & 4        & 0.21    &  & 176        & 768        & 4         & 0.28     &  & 176       & 768        & 4         & 0.28      \\
router             &  & 89      & 285      & 4       & 0.09       &  & 65        & 305       & 3        & 0.15    &  & 65         & 306        & 3         & 0.19     &  & 65        & 303        & 3         & 0.21      \\
voter              &  & 1838    & 8596     & 13      & 2.23       &  & 2133      & 10793     & 10       & 7.22    &  & 2068       & 10082      & 10        & 5.58     &  & 2053      & 10081      & 10        & 7.87      \\ \midrule
Improvement        &  &         &          &         &            &  & -13.65\%  & -27.62\%  & 30.74\%  &         &  & -10.73\%   & -24.52\%   & 34.29\%   &          &  & -9.44\%   & -24.00\%   & 35.86\%   &           \\
Total              &  &         &          &         & 58.40      &  &           &           &          & 565.39  &  &            &            &           & 377.33   &  &           &            &           & 452.53    \\ \bottomrule
\end{tabularx}
\end{table*}
